All Rivers Run to the Sea: Private Learning with Asymmetric Flows

Data privacy is of great concern in cloud machine-learning service platforms, when sensitive data are exposed to service providers. While private computing environments (e.g., secure enclaves), and cryptographic approaches (e.g., homomorphic encryption) provide strong privacy protection, their computing performance still falls short compared to cloud GPUs. To achieve privacy protection with high computing performance, we propose Delta, a new private training and inference framework, with comparable model performance as non-private centralized training. Delta features two asymmetric data flows: the main information-sensitive flow and the residual flow. The main part flows into a small model while the residuals are offloaded to a large model. Specifically, Delta embeds the information-sensitive representations into a low-dimensional space while pushing the information-insensitive part into high-dimension residuals. To ensure privacy protection, the low-dimensional information-sensitive part is secured and fed to a small model in a private environment. On the other hand, the residual part is sent to fast cloud GPUs, and processed by a large model. To further enhance privacy and reduce the communication cost, Delta applies a random binary quantization technique along with a DP-based technique to the residuals before sharing them with the public platform. We theoretically show that Delta guarantees differential privacy in the public environment and greatly reduces the complexity in the private environment. We conduct empirical analyses on CIFAR-10, CIFAR-100 and ImageNet datasets and ResNet-18 and ResNet-34, showing that Delta achieves strong privacy protection, fast training, and inference without significantly compromising the model utility.

==> fig/fig_sepback.tex <==
\begin{figure}[!htb]
    \centering
    \begin{tikzpicture}[node distance=1cm, auto,]
            \node[op, draw=black!30, fill=black!10, text width=8mm] (MR) {\scriptsize \IRR{}};
            \node[op, draw=red!30, fill=red!10, below=6mm of MR, text width=8mm ] (MM) {\scriptsize \IRM{}};
            \node[op, draw=black!30, fill=black!10,, right=3mm of MR, text width=8mm] (M2) {\scriptsize $\mathcal{M}_{\text{res}}$};
            \node[op, draw=red!30, fill=red!10, below=6mm of M2, text width=8mm] (M1) {\scriptsize $\mathcal{M}_{\text{main}}$};
            \node[op, draw=red!30, fill=red!10, right=10mm of M2, yshift=-5mm, text width=10mm] (softmax) {\scriptsize $\texttt{Softmax}$};
            % \node[left=3mm of MR, yshift=-4.5mm] (input) {\scriptsize Input};
            % \node[right=1mm of softmax] (output) {\scriptsize Output};
            \node[above=3mm of softmax, xshift=-1mm] (logits1) {\scriptsize with \MRS{}'s logits only};
            \node[below=3mm of softmax, xshift=1mm] (logits2) {\scriptsize with \MRS{}+\MM{}'s logits};
    
            % backward passes
            \draw[black!40, line width=0.5pt, ->]    (softmax.west) to [out=180, in=0] (M2.east);
            \draw[red!50, line width=1pt, ->]        (softmax.west) to [out=180, in=0] (M1.east);
            \draw[black!40, ->]                      (M2) to (MR);
            \draw[red!50, line width=1pt, ->]                        (M1) to (MM);
        \end{tikzpicture}
    \caption{The separate backpropagation on logits is illustrated. Gradients to \MRS{} are computed with \MRS{}'s own logtis only, therefore avoiding leaking logits of \MM{} to the outside.}
    \label{fig:sepback}
\end{figure}
